Learn-by-interact: A Data-Centric Framework for Self-Adaptive Agents in Realistic Environments

Autonomous agents powered by large language models (LLMs) have the potential to enhance human capabilities, assisting with digital tasks from sending emails to performing data analysis. The abilities of existing LLMs at such tasks are often hindered by the lack of high-quality agent data from the corresponding environments they interact with. We propose Learn-by-interact, a data-centric framework to adapt LLM agents to any given environments without human annotations. Learn-by-interact synthesizes trajectories of agent-environment interactions based on documentations, and constructs instructions by summarizing or abstracting the interaction histories, a process called backward construction. We assess the quality of our synthetic data by using them in both training-based scenarios and training-free in-context learning (ICL), where we craft innovative retrieval approaches optimized for agents. Extensive experiments on SWE-bench, WebArena, OSWorld and Spider2-V spanning across realistic coding, web, and desktop environments show the effectiveness of Learn-by-interact in various downstream agentic tasks -- baseline results are improved by up to 12.2\% for ICL with Claude-3.5 and 19.5\% for training with Codestral-22B. We further demonstrate the critical role of backward construction, which provides up to 14.0\% improvement for training. Our ablation studies demonstrate the efficiency provided by our synthesized data in ICL and the superiority of our retrieval pipeline over alternative approaches like conventional retrieval-augmented generation (RAG). We expect that Learn-by-interact will serve as a foundation for agent data synthesis as LLMs are increasingly deployed at real-world environments.

==> tables/data_samples/swebench.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{SWE-bench example} 
}
\begin{tabular}{p{13cm}}
\toprule
% \hspace{5.5cm} Biology \\
% \midrule
\textbf{Instruction} \\
\midrule
Please address the following Github issue. 
\bigbreak
\#\#\# GitHub Problem Description \#\#\# \\
ModelChoiceIteratorValue is not hashable. \\
Description
\bigbreak
Recently I migrated from Django 3.0 to Django 3.1. In my code, I add custom data-* attributes to the select widget options. After the upgrade some of those options broke. Error is {TypeError}unhashable type: 'ModelChoiceIteratorValue'. \\
Example (this one breaks): \\
\quad def create\_option(self, name, value, label, selected, index, subindex=None, attrs=None): \\
\quad \quad context = super().create\_option(name, value, label, selected, index, subindex, attrs) \\
\quad \quad if not value: \\
\quad \quad \quad return context \\
\quad \quad if value in self.show\_fields: \# This is a dict {1: ['first\_name', 'last\_name']} \\
\quad \quad \quad context['attrs']['data-fields'] = json.dumps(self.show\_fields[value]) \\
However, working with arrays is not an issue: \\
\quad def create\_option(self, name, value, label, selected, index, subindex=None, attrs=None): \\
\quad \quad context = super().create\_option(name, value, label, selected, index, subindex, attrs) \\
\quad \quad if not value: \\
\quad \quad \quad return context \\
\quad \quad if value in allowed\_values: \# This is an array [1, 2] \\
\quad \quad \quad ...\\
\midrule
\textbf{Observation 0 (repository structure)} \\
\midrule
django/ \\
\quad setup.py \\
\quad \_\_init\_\_.py \\
\quad \_\_main\_\_.py \\
\quad shortcuts.py \\
\quad forms/ \\
\quad \quad \_\_init\_\_.py \\
\quad \quad utils.py \\
\quad \quad fields.py \\
\quad \quad renderers.py \\
\quad \quad forms.py \\
\quad \quad formsets.py \\
% \quad \quad widgets.py \\
% \quad \quad boundfield.py \\
% \quad \quad models.py \\
% \quad db/ \\
% \quad \quad \_\_init\_\_.py \\
% \quad \quad transaction.py \\
% \quad \quad utils.py \\
% \quad \quad models/ \\
% \quad \quad \quad signals.py \\
% \quad \quad \quad constants.py \\
% \quad \quad \quad fields/ \\
% \quad \quad \quad \quad files.py \\
% \quad \quad \quad \quad \_\_init\_\_.py \\
% \quad \quad \quad \quad related.py \\
% \quad urls/ \\
% \quad \quad \_\_init\_\_.py \\
% \quad \quad converters.py \\
% \quad \quad exceptions.py \\
% \quad \quad base.py \\
% \quad \quad resolvers.py \\
% \quad \quad utils.py \\
% \quad \quad conf.py \\
% \quad middleware/ \\
% \quad \quad \_\_init\_\_.py \\
% \quad \quad common.py \\
% \quad \quad locale.py \\
% \quad \quad security.py \\
% \quad \quad csrf.py \\
% \quad \quad cache.py \\
% \quad \quad clickjacking.py \\
% \quad \quad http.py \\
% \quad \quad gzip.py \\
% \quad db/ \\
% \quad \quad \_\_init\_\_.py \\
% \quad \quad transaction.py \\
% \quad \quad utils.py \\
... \\
\bottomrule
\end{tabular}

\label{tab:swe_example_1}
\end{table}









\begin{table}[ht]
\caption{\textbf{SWE-bench example cont.}}
\centering
\begin{tabular}{p{13cm}}
\toprule
\textbf{Action 1 (Find related files to edit)} \\
\midrule
Based on the problem description and the repository structure, here are the most likely files that would need to be edited to fix the issue:
\bigbreak
django/forms/models.py \\
django/forms/fields.py \\
django/forms/widgets.py \\
django/forms/\_\_init\_\_.py \\
django/db/models/fields/\_\_init\_\_.py \\
django/db/models/fields/related.py \\
... \\
% django/core/exceptions.py \\
% django/utils/functional.py \\
% django/utils/hashable.py \\
% django/utils/\_\_init\_\_.py \\
\midrule
\textbf{Observation 1 (File skeleton)} \\
\midrule
\#\#\# File: django/forms/models.py \\
% \_\_all\_\_ = ( \\
% \quad `ModelForm', `BaseModelForm', `model\_to\_dict', \\
% \quad `fields\_for\_model', `ModelChoiceField', `ModelMultipleChoiceField' \\
% ) 
% \bigbreak
def construct\_instance(form, instance, fields=None, exclude=None): \\
\quad ... \\
% \bigbreak
def model\_to\_dict(instance, fields=None, exclude=None): \\
\quad ... \\
% \bigbreak
class ModelChoiceIteratorValue: \\
% \bigbreak
\quad def \_\_init\_\_(self, value, instance): \\
\quad \quad ... \\
% \bigbreak
\quad def \_\_str\_\_(self): \\
\quad \quad ... \\
% \bigbreak
\quad def \_\_eq\_\_(self, other): \\
\quad \quad ... \\
% \bigbreak
class ModelChoiceField(ChoiceField): \\
\quad def \_get\_choices(self): \\
\quad \quad ... \\
% \bigbreak
\#\#\# File: django/forms/fields.py \\
% \_\_all\_\_ = ( \\
%     `Field', `CharField', `IntegerField', \\
%     `DateField', `TimeField', `DateTimeField' \\
% )
% \bigbreak
class Field: \\
\quad widget = TextInput  \# Default widget to use when  rendering this type of Field. \\
\quad hidden\_widget = HiddenInput  \# Default widget to use when rendering this as "hidden"
\bigbreak
\quad def \_\_init\_\_(self, *, required=True, widget=None, label=None, initial=None): \\
\quad ... \\
\quad def prepare\_value(self, value): \\
\quad ... \\
\quad def to\_python(self, value): \\
\quad ... \\
\quad def validate(self, value): \\
\quad ... \\
% \quad def run\_validators(self, value): \\
% \quad ... \\
% class ChoiceField(Field): \\
% \quad def validate(self, value): \\
% \quad \quad ... \\
% \quad def valid\_value(self, value): \\
% \quad \quad ... \\
... \\
\bottomrule
\end{tabular}

\label{tab:swe_example_2}
\end{table}







\begin{table}[ht]
\caption{\textbf{SWE-bench example cont.}}
\centering
\begin{tabular}{p{13cm}}
\toprule
\textbf{Action 2 (Find related classes, methods to edit)} \\
\midrule
Here are the identified locations that need inspection or editing to fix the problem:
\bigbreak
django/forms/models.py \\
class: ModelChoiceIteratorValue
\bigbreak
% django/forms/models.py \\
% class: ModelChoiceField \\
% method: \_get\_choices
django/forms/models.py \\
class: ModelChoiceField \\
method: \_get\_choices
\bigbreak
django/forms/fields.py \\
class: ChoiceField \\
method: valid\_value \\

% django/forms/widgets.py
% class: Select
% method: create_option

% django/forms/widgets.py
% class: ChoiceWidget
% method: create_option

% django/forms/fields.py
% class: ChoiceField
% method: valid_value

% django/forms/fields.py
% class: TypedChoiceField
% method: _coerce

% django/forms/fields.py
% class: MultipleChoiceField
% method: to_python

% django/forms/fields.py
% class: TypedMultipleChoiceField
% method: _coerce
... \\
\midrule
\textbf{Observation 2 (Classes and methods content)} \\
\midrule
\#\#\# File django/forms/models.py \\
class ModelChoiceIteratorValue: \\
\quad def \_\_init\_\_(self, value, instance): \\
\quad \quad self.value = value \\
\quad \quad self.instance = instance
\bigbreak
\quad def \_\_str\_\_(self): \\
\quad \quad return str(self.value)
\bigbreak
\quad def \_\_eq\_\_(self, other): \\
\quad \quad if isinstance(other, ModelChoiceIteratorValue): \\
\quad \quad \quad other = other.value \\
\quad \quad return self.value == other \\
\bigbreak
% class ModelChoiceIterator: \\
% \quad def \_\_init\_\_(self, field): \\
% \quad \quad self.field = field \\
% \quad \quad self.queryset = field.queryset 
% \bigbreak
% \quad def \_\_bool\_\_(self): \\
% \quad \quad return self.field.empty\_label is not None or self.queryset.exists() 
% \bigbreak
% \quad def choice(self, obj): \\
% \quad \quad return ( \\
% \quad \quad \quad ModelChoiceIteratorValue(self.field.prepare\_value(obj), obj), \\
% \quad \quad \quad self.field.label\_from\_instance(obj), \\
% \quad \quad ) \\
% \bigbreak
class ModelChoiceField(ChoiceField):
\bigbreak
\quad def \_get\_choices(self): \\
\quad \quad return self.iterator(self)
\bigbreak
\#\#\# django/forms/fields.py \\
class ChoiceField(Field):
\bigbreak
% \quad def \_\_init\_\_(self, *, choices=(), **kwargs): \\
% \quad \quad super().\_\_init\_\_(**kwargs) \\
% \quad \quad self.choices = choices 
% \bigbreak
\quad def valid\_value(self, value): \\
\quad \quad text\_value = str(value) \\
\quad \quad for k, v in self.choices: \\
\quad \quad \quad if isinstance(v, (list, tuple)): \\
\quad \quad \quad \quad \# This is an optgroup, so look inside the group for options \\
% \quad \quad \quad \quad for k2, v2 in v: \\
% \quad \quad \quad \quad \quad if value == k2 or text\_value == str(k2): \\
% \quad \quad \quad \quad \quad \quad return True \\
% \quad \quad \quad else: \\
% \quad \quad \quad \quad if value == k or text\_value == str(k): \\
% \quad \quad \quad \quad \quad return True \\
% \quad \quad return False \\
... \\
\bottomrule
\end{tabular}

\label{tab:swe_example_3}
\end{table}


\begin{table}[ht]
\caption{\textbf{SWE-bench example cont.}}
\centering
\begin{tabular}{p{13cm}}
\toprule
\textbf{Action 3 (Edit code to address the issue)} \\
\midrule
Based on the issue description and the provided code segment, it appears that the `ModelChoiceIteratorValue` class is not hashable, which is causing the TypeError when trying to use it as a dictionary key. To fix this, we need to make the `ModelChoiceIteratorValue' class hashable by implementing the `\_\_hash\_\_' method. Here's the proposed fix:
\bigbreak
\#\#\# django/forms/models.py \\
\#\#\# Replace the following code \\
class ModelChoiceIteratorValue: \\
\quad def \_\_init\_\_(self, value, instance): \\
\quad \quad self.value = value \\
\quad \quad self.instance = instance
\bigbreak
\quad def \_\_str\_\_(self): \\
\quad \quad return str(self.value)
\bigbreak
\quad def \_\_eq\_\_(self, other): \\
\quad \quad if isinstance(other, ModelChoiceIteratorValue): \\
\quad \quad \quad other = other.value \\
\quad \quad return self.value == other
\bigbreak
\#\#\# with
\bigbreak
class ModelChoiceIteratorValue: \\
\quad def \_\_init\_\_(self, value, instance): \\
\quad \quad self.value = value \\
\quad \quad self.instance = instance
\bigbreak
\quad def \_\_str\_\_(self): \\
\quad \quad return str(self.value)
\bigbreak
\quad def \_\_eq\_\_(self, other): \\
\quad \quad if isinstance(other, ModelChoiceIteratorValue): \\
\quad \quad \quad other = other.value \\
\quad \quad return self.value == other
\bigbreak
\quad def \_\_hash\_\_(self): \\
\quad \quad return hash(self.value) \\
\midrule
\textbf{Observation 3 (Generated patch)} \\
\midrule
diff --git a/django/forms/models.py b/django/forms/models.py \\
index 5a30801..55b3c81 100644 \\
- - - a/django/forms/models.py \\
+++ b/django/forms/models.py \\
@@ -1171,6 +1171,9 @@ class ModelChoiceIteratorValue: \\
\quad \quad \quad other = other.value \\
\quad \quad return self.value == other
\bigbreak 
+    def \_\_hash\_\_(self): \\
+        return hash(self.value) \\
+
\bigbreak 
class ModelChoiceIterator: \\
\quad def \_\_init\_\_(self, field): \\
\bottomrule
\end{tabular}

\label{tab:swe_example_4}
\end{table}



==> tables/task_specific_approach.tex <==
\begin{table}[t!]
\caption{Top-10 results of SWE-bench from the leaderboard at \url{https://www.swebench.com/}. All the numbers are fetched on 2024-10-01.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|c}
\toprule
Approach $\downarrow$ & site & result \\
\midrule
CodeStory Aide + Mixed Models & \url{https://www.swebench.com/} & 43.0 \\
Honeycomb & \url{https://honeycomb.sh/} & 38.3 \\
AbanteAI MentatBot & \url{https://mentat.ai/blog/mentatbot-sota-coding-agent} & 38.0 \\
Gru & \url{https://gru.ai/} & 35.7 \\
Isoform & \url{https://www.isoform.ai/} & 35.0 \\
SuperCoder2.0 & \url{https://superagi.com/supercoder/} & 34.0 \\
MarsCode & \url{https://www.marscode.com/} & 34.0 \\
Lingma & \url{https://arxiv.org/abs/2406.01422} & 33.0 \\
Factory Code Droid & \url{https://www.factory.ai/} & 31.3 \\
AutoCodeRover & \url{https://autocoderover.dev/} & 30.7 \\
\ours (ours) & This paper & 34.7 \\
\bottomrule
\end{tabular}

}
\label{tab:task_specific}
\end{table}






\begin{table}[t!]
\caption{Top-10 results of WebArena from the leaderboard at \url{https://docs.google.com/spreadsheets/d/1M801lEpBbKSNwP-vDBkC_pF7LdyGU1f_ufZb_NWNBZQ/edit?gid=0\#gid=0}. All the numbers are fetched on 2024-10-01.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|c}
\toprule
Approach $\downarrow$ & site & result \\
\midrule
Jace.AI & \url{https://www.jace.ai/} & 57.1 \\
WebPilot & \url{https://www.arxiv.org/pdf/2408.15978} & 37.2 \\
AWM & \url{https://arxiv.org/pdf/2409.07429} & 35.5 \\
Step & \url{https://arxiv.org/abs/2310.03720} & 33.5 \\
BrowserGym & \url{https://github.com/ServiceNow/BrowserGym} & 23.5 \\
Auto Eval & \url{https://arxiv.org/abs/2404.06474} & 20.2 \\
Tree Search & \url{https://jykoh.com/search-agents} & 19.2 \\
AutoWebGLM & \url{https://arxiv.org/abs/2404.03648} & 18.2 \\
gpt-4-0613 & \url{https://arxiv.org/abs/2307.13854} & 14.9 \\
gpt-4o-2024-05-13 & \url{https://arxiv.org/abs/2307.13854} & 13.1 \\
\ours (ours) & This paper & 39.2 \\
\bottomrule
\end{tabular}

}
\label{tab:task_specific_1}
\end{table}





